Measurement of Branching Fraction and Time-Dependent CP Asymmetry Parameters in B0 -> D*+ D*- Ks Decays

We present a measurement of the branching fraction and time-dependent CP violation parameters for B0 -> D*+ D*- Ks decays. We also obtain an upper limit on the product branching fraction for the possible two-body decay, B0 -> Ds1+(2536) D*-. These results are obtained from a 414 fb-1 data sample that contains 449e10^6 BBbar pairs collected at the Upsilon(4S) resonance with the Belle detector at the KEKB asymmetric e+e- collider.

==> abstract.tex <==
We present a measurement of the branching fraction and time-dependent CP violation parameters for B0 -> D*+ D*- Ks decays. We also obtain an upper limit on the product branching fraction for the possible two-body decay, B0 -> Ds1+(2536) D*-. These results are obtained from a 414 fb-1 data sample that contains 449e10^6 BBbar pairs collected at the Upsilon(4S) resonance with the Belle detector at the KEKB asymmetric e+e- collider.

